Misspecified Recovery

Asset prices contain information about the probability distribution of future states and the stochastic discounting of those states as used by investors. To better understand the challenge in distinguishing investors' beliefs from risk-adjusted discounting, we use Perron-Frobenius Theory to isolate a positive martingale component of the stochastic discount factor process. This component recovers a probability measure that absorbs long-term risk adjustments. When the martingale is not degenerate, surmising that this recovered probability captures investors' beliefs distorts inference about risk-return tradeoffs. Stochastic discount factors in many structural models of asset prices have empirically relevant martingale components.

==> defs_paper_11pt.tex <==
% packages for inclusion

\usepackage{sectsty}
\usepackage{amsmath,amssymb,amsthm,enumerate,graphicx}
\usepackage{ifthen,latexsym,syntonly}
\usepackage{setspace}
\usepackage[normalem]{ulem}
\usepackage{cancel}
%\usepackage[showrefs]{refcheck}  %use this to show equation and section labels
\usepackage{color}
\usepackage[round,comma,authoryear]{natbib}
%\usepackage{pstricks}
\usepackage{pgfplots}

%\usepackage{refcheck}

%\usepackage{mathtools}
%\mathtoolsset{showonlyrefs}

% for natbib
%\usepackage{subfigure}
\bibliographystyle{mynat}
%\bibliographystyle{jpe}

\onehalfspacing

% for natbib
%\bibpunct{(}{)}{,}{a}{}{,}  % for natbib
%                            % need to have mynat.bst in an accessible directory

\bibpunct{(}{)}{,}{a}{}{,}  % for natbib
                            % need to have mynat.bst in an accessible directory

%\usepackage{refcheck}

\ifthenelse{\isundefined{\theorem}}
{
\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
%\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{Restriction}[theorem]{Restriction}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{result}[theorem]{Result}
%\newtheorem{solution}[theorem]{Solution}
%\newtheorem{summary}[theorem]{Summary}
\newtheorem{thm}[theorem]{Theorem}
}{}

\newenvironment{exampleenv}[1][Exampleenv]{\noindent\begin{example}}{\makebox[1em][l]{} \hspace{-1em} \hfill $\Box$\end{example}}


% =======================================================================
%\setlength{\oddsidemargin}{0in} \setlength{\topmargin}{0in}
%\setlength{\textwidth}{6.5in} \setlength{\textheight}{8.5in}

\setlength{\voffset}{0in} \setlength{\topmargin}{0in}
\setlength{\headheight}{0in} \setlength{\headsep}{0in}
\setlength{\textheight}{9in}
\setlength{\hoffset}{0in} \setlength{\oddsidemargin}{0in}
\setlength{\evensidemargin}{0cm}
\setlength{\textwidth}{6.5in}

% =======================================================================
% special letters
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\E}{\mathcal{E}}


% ===========================================================
% hypertext links

\usepackage[breaklinks]{hyperref} % dvips options switched off
\usepackage{ifthen}

% hyperref definitions for citation and reference linking
% options pdfpagemode=FullScreen - after PDF opens, it goes to fullscreen
\hypersetup{pdfpagemode=UseNone, colorlinks=true, anchorcolor=webbrown, citecolor=webbrown, filecolor= webbrown, linkcolor= webbrown, menucolor= webbrown,
urlcolor= webbrown, citebordercolor=1 0 0, menubordercolor=1 0 0, urlbordercolor=1 0 0, runbordercolor=1 0 0}
\definecolor{webgreen}{rgb}{0,.5,0}
\definecolor{webbrown}{rgb}{.6,0,0}
\definecolor{webblue}{rgb}{0,0,0.8}
\definecolor{webpurple}{rgb}{0.7,0,0.7}

% ===========================================================
% draft notes
\usepackage{version}
\ifthenelse{\isundefined{\draftnote}}{\newenvironment{draftnote}[1][Draft note]{}{}}{}
\ifthenelse{\isundefined{\includedraftnotes}}{\def\includedraftnotes{false}}{}

\ifthenelse{\equal{\includedraftnotes}{true}}{%
  \renewenvironment{draftnote}[1][Draft note:]%
    {\vspace{2mm}\addtolength{\leftskip}{10mm}\addtolength{\rightskip}{10mm}\begin{small}\noindent\textbf{#1}\ \ }%
    {\hfill\rule{0.5em}{0.5em}\end{small}\par\vspace{2mm}}
}{
  \renewenvironment{draftnote}[1][Draft note:]{}{}
  \excludeversion{draftnote}
}

% ===========================================================
\usepackage{subfiles}
% the following makes sure that packages are not read in subfiles
\ifthenelse{\isundefined{\ssubfile}}{\def\ssubfile{yes}}{}


% ===========================================================
% definition of the title

\ifthenelse{\isundefined{\mmaketitle}}{\def\mmaketitle{false}}{}
\ifthenelse{\isundefined{\ttitle}}{\def\ttitle{}}{}
\ifthenelse{\isundefined{\ttitlefootnote}}{\def\ttitlefootnote{}}{}
\ifthenelse{\isundefined{\aauthor}}{\def\aauthor{}}{}
\ifthenelse{\isundefined{\aauthorfootnote}}{\def\aauthorfootnote{}}{}
\ifthenelse{\isundefined{\aauthorinstitution}}{\def\aauthorinstitution{}}{}
\ifthenelse{\isundefined{\aauthoremail}}{\def\aauthoremail{}}{}
\ifthenelse{\isundefined{\ddate}}{\def\ddate{}}{}
\ifthenelse{\isundefined{\aabstract}}{\def\aabstract{}}{}
\ifthenelse{\isundefined{\pprintcontents}}{\def\pprintcontents{false}}{}
\ifthenelse{\isundefined{\separatefrontmatterpages}}{\def\separatefrontmatterpages{false}}{}

% symbol footnotes
\newcommand{\symbolfootnote}[2][1]{%
  \renewcommand{\thefootnote}{\fnsymbol{footnote}}%
  \thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}%
}

% ===========================================================
% title page

\ifthenelse{\not\equal{\ttitle}{}}{%
  \ifthenelse{\not\equal{\ttitlefootnote}{}}{%
    \title{{\huge\ttitle}\thanks{\ttitlefootnote}\vspace{5mm}}%
  }{%
    \title{{\huge\ttitle}\vspace{5mm}}%
  }%
}{}%
%\title{{\LARGE \ttitle}\thanks{\ttitlefootnote}}

\ifthenelse{\isundefined{\aauthorA}}{}{%
\ifthenelse{\not\equal{\aauthorA}{}}{%
  \newcommand{\aauthorsA}{{\Large\aauthorA}\vspace{3mm}\\
  {\large\begin{tabular}{c}\aauthorAinstitution \vspace{1mm} \\ \color{webbrown}\aauthorAemail\end{tabular}}}%
  \author{\aauthorsA\vspace{5mm}}%
}{}}%
%\ifthenelse{\isundefined{\aauthorB}}{}{%
%\ifthenelse{\not\equal{\aauthorB}{}}{%
%  \newcommand{\aauthorsAB}{\aauthorsA \and {\large\aauthorB} \\ %\begin{tabular}{c}\aauthorBinstitution\end{tabular} \\ \aauthorBemail}%
%  \author{\aauthorsAB\vspace{5mm}}
%}{}}%
\ifthenelse{\isundefined{\aauthorB}}{}{%
\ifthenelse{\not\equal{\aauthorB}{}}{%
  \newcommand{\aauthorsAB}{\aauthorsA \and {\Large\aauthorB} \vspace{3mm}\\ {\large\begin{tabular}{c}\aauthorBinstitution \vspace{1mm} \\ \color{webbrown}\aauthorBemail\end{tabular}}}%
  \author{\aauthorsAB\vspace{5mm}}%
}{}}%
\ifthenelse{\isundefined{\aauthorC}}{}{%
\ifthenelse{\not\equal{\aauthorC}{}}{%
  \newcommand{\aauthorsABC}{\aauthorsAB \and {\Large\aauthorC} \vspace{3mm}\\ {\large\begin{tabular}{c}\aauthorCinstitution \vspace{1mm} \\ \color{webbrown}\aauthorCemail\end{tabular}}}%
  \author{\aauthorsABC\vspace{5mm}}%
}{}}%

\date{\vspace{3mm}{\Large\ddate}}

\newcommand{\mmmaketitle}{%
  \ifthenelse{\equal{\mmaketitle}{true}}{%
    \maketitle
    \vspace{-10mm}
    \ifthenelse{\equal{\includedraftnotes}{true}}{%
      \begin{center}{\large Draft with notes. Not for distribution.}\end{center}\par \vspace{5mm}%
    }{}%
    \vfill

    \begin{abstract}
      \aabstract
    \end{abstract}
    \vfill%\vspace{5mm}
    \ifthenelse{\equal{\separatefrontmatterpages}{true}}{%
      \thispagestyle{empty}\setcounter{page}{0}
      \newpage%
    }{}%
    \ifthenelse{\equal{\pprintcontents}{true}}{%
      \thispagestyle{empty}
      {\setlength{\baselineskip}{0.8\baselineskip}\tableofcontents}%
      \ifthenelse{\equal{\separatefrontmatterpages}{true}}{%
        \thispagestyle{empty}\setcounter{page}{0}
        \newpage%
      }{}%
    }{}%
  }{}%
}



==> todolist.tex <==
% !TEX root = recovery_theorem_main1.tex



{\Large\bf\noindent TO DO LIST. Remove the link to this from main file before submitting.}

%{\bf From the referee report}
%
%\begin{enumerate}

%\item The following key paragraph in the introduction seems awkward:  In this
%paper we delineate the connection between these seemingly disparate
%results. We make clear the special assumptions that are needed to
%guarantee that the transition probabilities recovered using
%Perron–Frobenius Theory are equal to the subjective transition
%probabilities of investors or to the actual probabilities under an
%assumption of rational expectations. An extension of the Perron–Frobenius
%approach to include seemingly unnecessary state variables avoids the
%degeneracy in the implied long-term risk-return tradeoff. Unfortunately,
%full identification of the subjective beliefs is no longer feasible."
%
%There is no context for the "extension" sentences at the end. Moreover,
%before you get to this extension you do much more that strikes me as
%every bit as central to the paper. You not only make clear the special
%assumptions needed, you also provide salient economic settings where this
%recovery is not obtained and provide illustrative calibrated examples
%where actual probabilities are not obtained. Maybe you could play this up
%and leave off the last two sentences until you describe Section 8?
%
%{\color{red}Confirm Jos\'{e}'s modification.  LPH made some minor edits. Jarda confirms.}
%
%\item As for Section 8, why should a reader care that you can avoid the
%degenerate long-term risk-return trade-off? Presumably because there are
%interesting modeling or economic questions that lead one to explore this
%extension? Why not open in your introduction with a more practical
%motivation like: some might wonder whether the presence of a martingale
%component is splitting hairs between a highly persistent stationary
%process and a non-stationary process. Well we show that identification
%can become tenuous when the state-vector is extended to address this
%"approximation issue."
%
%{\color{red}Confirm Jos\'{e}'s modification.}

% \item Page 12: "the analysts attributes" should be "the analyst attributes"

%\item Page 13 typo "examples thas we provide later"

%\item Page 14: This sentence is not easily interpreted: To include this richer
%collection of models, we allow our multiplicative functional to depend on
%a shock vector  $\Delta W$ that is the normally distributed shock vector
%and hence not fully revealed by the evolution of the state X. Why is
%this âthe⠀ normally distributed shock vector? Do you mean "depend on the
%normally distributed shock vector $\Delta W$ that is not fully revealed
%by..."?
%
%{\color{red}Confirm Jos\'{e}'s modification. LPH fine.}

%\item If you have not already done so, please read the JF's Conflict of
%Interest Disclosure Policy and provide a Disclosure Statement from each
%author.
%
%The final version of your paper should integrate your disclosure
%statements into your manuscript as follows: If the disclosure statement
%is brief, it should be included in the "acknowledgments" footnote. If the
%disclosure statement is longer, then disclosure will have two parts: (i)
%a brief statement summarizing potential conflicts of interest that will
%be included in the "acknowledgments" footnote; (ii) a more detailed
%description of the activities and relationships that are the source of a
%potential conflict of interest. This more detailed account will be
%available to the public. The "acknowledgments" footnote will include a
%pointer/link to the detailed electronic version of the disclosure
%statement which will be archived on the journal's website.
%
%{\color{red}Confirm acknowledgements.  LPH fine.}

%\end{enumerate}

{\bf Other comments}

\begin{enumerate}

%\item The abstract should be doublespaced and have no more than 100 words (right now, we have 173).

\item Check JEL classification and keywords.

%item Check that we are not missing equation numbers.

\item Should we include Schneider and Trojani, (and Martin) on the lower bound of expected returns? It's conceptually different (they rely on time-series information) but the former uses the divergence measures.

%\item I added the disclosure statement in line with what each of us wrote. It is in the acknowledgement. Please check it. I added NYU to mine to be in line with Jos\'{e}.

\end{enumerate}

%General Text
%\begin{enumerate}
%\item Text must be in literary present tense throughout. For example, "we predict the dependent
%variable" rather than "we predicted the dependent variable." Use past tense when describing
%historical events. For example, "investors sold shares in our sample" rather than "investors sell
%shares in our sample."
%\item Grammar, spelling, and punctuation corrections must be made.
%\item Do not start a sentence with notation (i.e., variables).
%\item Adverb phrases do not need to be hyphenated (e.g., actively managed, not actively-managed).
%\item Bullet points or small roman numerals (e.g., (i), (ii), etc.) may be used to list items.
%\item Please use the following treatment: ``See, for example, ...'' rather than ``See, e.g., ....'' Similarly,
%use ``..., that is, .....'' rather than ``..., i.e., .....'' However, ``(i.e., ...)'' or ``(e.g., ...)'' is fine.
%\item Do not use italics on Latin. For example, ``ceteris paribus'' rather than ``ceteris paribus.''
%\end{enumerate}

%Figures
%\begin{enumerate}
%%\item Figures are numbered with Arabic numerals and must have a caption. There should also be a
%%descriptive legend if necessary to explain what the figure shows or to define variable notation (as
%%with tables, figure legends should direct the reader to a separate definitions table or appendix if
%%lengthy, OR to a previous figure as appropriate).
%%\item Indicate the location of the figures in the margin of the paper's text.
%%\item Figures must be camera-ready with all axes labeled.
%\item If you want to use color in figures, contact Wendy Washburn at editor@jfinance.org about
%getting a cost estimate from the publisher; otherwise, convert any color to grayscale.
%\end{enumerate}

